SemEval-2020 Task 7: Assessing Humor in Edited News Headlines

This paper describes the SemEval-2020 shared task "Assessing Humor in Edited News Headlines." The task's dataset contains news headlines in which short edits were applied to make them funny, and the funniness of these edited headlines was rated using crowdsourcing. This task includes two subtasks, the first of which is to estimate the funniness of headlines on a humor scale in the interval 0-3. The second subtask is to predict, for a pair of edited versions of the same original headline, which is the funnier version. To date, this task is the most popular shared computational humor task, attracting 48 teams for the first subtask and 31 teams for the second.

==> bk-results-baselines-copy.tex <==
\renewcommand{\arraystretch}{0.88}
\begin{tabular}{@{}l|crc|crrc@{}}
\toprule
{} & \multicolumn{3}{c}{\textbf{Subtask 1}} & \multicolumn{4}{c}{\textbf{Subtask 2}} \\ \textbf{Model} & \textbf{RMSE$^\dagger$} & \textbf{Gain} & \textbf{Spearman} & \textbf{Accuracy$^\dagger$} & \textbf{Gain} & \textbf{Reward} & \textbf{RMSE} \\
\midrule
Baseline & 0.575 & -0.033 & / & 0.490 & -0.109 & -0.020 & / \\
\midrule
CBOW &&&&&&& \\
\quad with \textsc{Context}+\textsc{Freeze} & \textbf{0.542} & \textbf{0.000} & \textbf{0.319} & 0.599 & 0.000 & 0.184 & 0.546 \\
\quad +\textsc{Original} & 0.559 & -0.017 & 0.243 & 0.599 & 0.000 & 0.169 & 0.760 \\
\quad +\textsc{Extra} & 0.544 & -0.002 & 0.308 & 0.605 & 0.006 & \textbf{0.191} & \textbf{0.545} \\
\quad +\textsc{Original}+\textsc{Extra} & 0.558 & -0.016 & 0.250 & 0.601 & 0.002 & 0.173 & 0.574 \\
\quad +FT & 0.544 & -0.002 & 0.311 & 0.604 & 0.005 & 0.178 & \textbf{0.545} \\
\quad +FT+\textsc{Original} & 0.561 & -0.019 & 0.247 & 0.592 & -0.007 & 0.165 & 0.604 \\
\quad +FT+\textsc{Extra} & 0.548 & -0.006 & 0.313 & \textbf{0.606} & \textbf{0.007} & 0.188 & 0.547 \\
\quad +FT+\textsc{Original}+\textsc{Extra} & 0.563 & -0.021 & 0.261 & 0.589 & -0.010 & 0.161 & 0.581 \\
\midrule
BERT &&&&&&& \\
\quad with \textsc{Context}+\textsc{Freeze} & 0.531 & 0.011 & 0.384 & 0.616 & 0.017 & 0.207 & 0.546 \\
\quad +\textsc{Original} & 0.534 & 0.008 & 0.366 & 0.603 & 0.004 & 0.186 & 0.547 \\
\quad +\textsc{Extra} & \textbf{0.530} & \textbf{0.012} & 0.382 & 0.615 & 0.016 & 0.207 & \textbf{0.530} \\
\quad +\textsc{Original}+\textsc{Extra} & 0.541 & 0.001 & 0.346 & 0.615 & 0.016 & 0.204 & 0.542 \\
\quad +FT & 0.536 & 0.006 & 0.366 & \textbf{0.635} & \textbf{0.036} & 0.234 & 0.552 \\
\quad +FT+\textsc{Original} & 0.536 & 0.006 & 0.365 & 0.628 & 0.029 & 0.231 & 0.555 \\
\quad +FT+\textsc{Extra} & 0.541 & 0.001 & 0.373 & 0.630 & 0.031 & 0.232 & 0.554 \\
\quad +FT+\textsc{Original}+\textsc{Extra} & 0.533 & 0.009 & \textbf{0.387} & 0.629 & 0.030 & \textbf{0.236} & 0.550 \\
\midrule
RoBERTa &&&&&&& \\
\quad with \textsc{Context}+\textsc{Freeze} & 0.528 & 0.014 & 0.388 & 0.635 & 0.036 & 0.246 & \underline{\textbf{0.529}} \\
\quad +\textsc{Original} & 0.536 & 0.006 & 0.366 & 0.625 & 0.026 & 0.224 & 0.540 \\
\quad +\textsc{Extra} & 0.528 & 0.014 & 0.390 & 0.640 & 0.041 & 0.252 & 0.536 \\
\quad +\textsc{Original}+\textsc{Extra} & 0.533 & 0.009 & 0.368 & 0.618 & 0.019 & 0.207 & 0.543 \\
\quad +FT & 0.534 & 0.008 & 0.382 & 0.649 & 0.050 & \underline{\textbf{0.254}} & 0.535 \\
\quad +FT+\textsc{Original} & 0.527 & 0.015 & \underline{\textbf{0.425}} & \underline{\textbf{0.650}} & \underline{\textbf{0.051}} & \underline{\textbf{0.254}} & 0.538 \\
\quad +FT+\textsc{Extra} & 0.526 & 0.016 & 0.407 & 0.638 & 0.039 & 0.233 & 0.594 \\
\quad +FT+\textsc{Original}+\textsc{Extra} & \underline{\textbf{0.522}} & \underline{\textbf{0.020}} & 0.410 & 0.626 & 0.027 & 0.216 & 0.625 \\
\bottomrule
\end{tabular}

==> bksec4.tex <==
\section{Evaluation}

\subsection{Metrics}
For Subtask 1, systems are ranked using the root mean squared error (RMSE) between the mean of the five annotators' ratings and the rating predicted by the system for the headline:

$$RMSE = \sqrt{\frac{\sum^N_{i=1} (y_i -\hat{y_i})^2}{N}} $$

\noindent where $N$ is the size of the test set, and $y_i$ and $\hat{y_i}$ are, respectively, the ground truth and the predicted labels for the $i$-th sample.  Additionally, we report the RMSE obtained by considering only the $X\%$ most funny headlines and $X\%$ least funny headlines in the test set, for $X \in \{10,20,30,40\}$.  \nh{call this `bucket performance metric' as stated by YNU-HPCC?}

For Subtask 2, which attempts to find the funniest of two headlines, the evaluation metric is classification accuracy. Given $N$ test samples with $C$ correct predictions:

$$ Accuracy = \frac{C}{N} $$ % \times 100\% $$

\noindent We ignore cases where the two edited versions of a headline have the same ground truth mean funniness. We report another auxiliary metric called the reward: $r = \frac{1}{N}\sum^N_{i=1}(\mathbbm{1}_{\hat{y_i}=y_i} - \mathbbm{1}_{\hat{y_i}\neq y_i})|z_i^{(1)}-z_i^{(2)}| $. The larger the funniness difference between the two headlines in the pair, higher is the reward (or penalty) for a correct classification (or misclassification). \nh{Explain motivations?}

%\usage{We also report the system reward. The pair-wise reward is the positive (or negative) difference between the ratings of the two edited headline versions for a correct (or wrong) prediction. The system reward is the mean of all pair-wise rewards (we ignore cases where the two edited versions of a headline have the same ground truth mean funniness).}

\subsection{Baselines}
We provide several baselines in Table~\ref{tab:baseline} to compare against participating systems:\footnote{reproduced with permission from the Duluth team~\cite{duluth2020semeval}, who performed these exhaustive experiments.} 
\begin{enumerate}%[leftmargin=*]
\itemsep-0.1em 
    \item Na\"ive Baseline: assigns the mean grade (Subtask 1) or the majority label (Subtask 2) from the training set. \nh{Call it Trivial as people may confuse Naive with Naive Bayes?}
    \item CBOW: the context independent continuous bag of words model obtained using the pretrained GloVe word vectors with 300d embeddings and a dictionary of 2.2M words from Common Crawl. 
    \item BERT: the bert-base-uncased model ($L = 12$, $d = 768$, lower-cased)
    \item RoBERTa: the roberta-base model ($L = 12$, $d = 768$)
\end{enumerate}
\noindent Each neural baseline result uses the edited headline. Additionally, C{\small ONTEXT} implies using the headline's context (the replaced word substituted with \texttt{MASK}), O{\small RIGINAL} implies using the original headline, FT refers to finetuning, F{\small REEZE} implies feature extraction (no finetuning) and E{\small XTRA} refers to using the FunLines training data. For a thorough discussion of these baseline implementations, we refer the reader to~\cite{duluth2020semeval}.

The results for Subtask 2 were obtained by using the model trained for Subtask 1 to assign funniness ratings to both the edited versions of a headline and then choosing the version scoring higher.

\begin{table}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/baseline.png}
    \caption{Baselines on the test set. F{\small REEZE}: no finetuning; FT: finetuning; C{\small ONTEXT}: use context of edited headline; O{\small RIGINAL}: use original headline; E{\small XTRA}: use additional training data from the FunLines dataset. \textbf{RMSE$^\dagger$} and \textbf{Accuracy$^\dagger$} are primary metrics. The best within each model type is bolded, and the overall best ins \underline{underlined}. Gain measures the improvement (in RMSE or accuracy) over CBOW-C{\small ONTEXT}-F{\small REEZE}. Baseline for Subtask 1 uses the mean grade and Baseline for Subtask 2 uses the majority label from the training set.  }
    \label{tab:baseline}
\end{table}


Table~\ref{tab:baseline} suggests that contextual information is useful in our humor recognition tasks, since the context independent GloVe embeddings (CBOW) lead to weaker performance compared to that achieved using the context-sensitive pre-trained BERT and RoBERTa embeddings. \nh{Does this belong in a later discussion section?}


%\setlength{\columnsep}{1pt}%
\begin{wraptable}{r}{0.39\textwidth}
    \centering
    \resizebox{0.38\textwidth}{!}{
    \begin{tabular}{|c|l|c|}
    \textbf{Rank}  & \textbf{Team}   & \textbf{RMSE} \\ \hline
    %\textbf{--} & \textbf{Na\"ive Baseline} & \textbf{0.57471} & \textbf{0.98616} & \textbf{0.83064} & \textbf{0.72266}	& \textbf{0.64004} & \textbf{0.00723} \\ \hline 

1  &  Hitachi  &  0.49725 \\ \hline
2  &  Amobee  &  0.50726 \\ \hline
3  &  YNU-HPCC  &  0.51737 \\ \hline
4  &  MLEngineer  &  0.51966 \\ \hline
5  &  LMML  &  0.52027 \\ \hline
6  &  ECNU  &  0.52187 \\ \hline
7  &  LT3  &  0.52532 \\ \hline
8  &  WMD  &  0.52603 \\ \hline
9  &  Ferryman  &  0.52776 \\ \hline
10  &  zxchen  &  0.52886 \\ \hline
11  &  Duluth  &  0.53108 \\ \hline
12  &  will\_go  &  0.53228 \\ \hline
13  &  XSYSIGMA  &  0.53308 \\ \hline
14  &  LRG  &  0.53318 \\ \hline
15  &  MeisterMorxrc  &  0.53383 \\ \hline
16  &  JUST\_Farah  &  0.53396 \\ \hline
17  &  Lunex  &  0.53518 \\ \hline
18  &  unituebingenCL  &  0.53954 \\ \hline
19  &  IRLab\_DAIICT  &  0.54670 \\ \hline
20  &  O698  &  0.54754 \\ \hline
21  &  UPB  &  0.54803 \\ \hline
22  &  Buhscitu  &  0.55115 \\ \hline
23  &  Fermi  &  0.55226 \\ \hline
24  &  INGEOTEC  &  0.55391 \\ \hline
25  &  JokeMeter  &  0.55791 \\ \hline
26  &  testing  &  0.55838 \\ \hline
27  &  HumorAAC  &  0.56454 \\ \hline
28  &  ELMo-NB  &  0.56829 \\ \hline
29  &  prateekgupta2533  &  0.56983 \\ \hline
30  &  funny3  &  0.57237 \\ \hline
31  &  WUY  &  0.57369 \\ \hline
32  &  XTHL  &  0.57470 \\ \hline
\textbf{--} & \textbf{Na\"ive Baseline} & \textbf{0.57471} \\ \hline 
33  &  HWMT\_Squad  &  0.57471 \\ \hline
34  &  moonalasad  &  0.57479 \\ \hline
35  &  dianehu  &  0.57488 \\ \hline
36  &  Warren  &  0.57527 \\ \hline
37  &  tangmen  &  0.57768 \\ \hline
38  &  Lijunyi  &  0.57946 \\ \hline
39  &  Titowak  &  0.58157 \\ \hline
40  &  xenia  &  0.58286 \\ \hline
41  &  Hahackathon  &  0.59202 \\ \hline
42  &  KdeHumor  &  0.61643 \\ \hline
43  &  uir  &  0.62401 \\ \hline
44  &  SO  &  0.65099 \\ \hline
45  &  heidy  &  0.68338 \\ \hline
46  &  Hasyarasa  &  0.70333 \\ \hline
47  &  frietz58  &  0.72252 \\ \hline
48  &  SSN\_NLP  &  0.84476 \\ \hline
    \end{tabular}}
    \caption{Official results for Subtask 1.}
    \label{tab:res-A}
\end{wraptable}

\subsection{Results}
The official results for Subtasks 1 and 2 are, respectively, in Tables~\ref{tab:res-A} and~\ref{tab:res-B}. There were 48 participants for Subtask 1. Subtask 2 attracted 31 participants, all of whom were also participants in Subtask 2 except UTFPR which only participated in Subtask 2. The best system in Subtask 1 was Hitachi, achieving an RMSE of 0.49725, a 13.5\% improvement over the Na\"ive baseline. The best performing system for Subtask 2, again Hitachi, achieved a classification accuracy of 67.43\%, far above the Na\"ive baseline's accuracy of 49.50\%. These results do not include the results from Team \emph{oyx}, who submitted results just after the evaluation phase ended, achieving 0.50157 RMSE for Subtask 1 and 67.24\% accuracy for Subtask 2. In total, the test phase attracted 50 participating teams.

%\nh{mention number of people who signed up for the task? Mention the number who submitted results on the dev set?}
\nh{Results indicate that just by flipping output label, the worst performer for Subtask 2 can achieve winning accuracy of 67.96\%. Could that be interesting? How can we be more space efficient for Table 2, flip it 90 degrees?}

\nh{Can report average performance gain using FunLines data for Subtasks 1 and 2}




\begin{wraptable}{r}{0.55\textwidth}
    \centering
    \resizebox{0.54\textwidth}{!}{
    %\begin{adjustbox}{angle=90}
    \begin{tabular}{|c|l|c|c|}
    \hline \textbf{Rank}  & \textbf{Team}   & \textbf{Accuracy}    & \textbf{Reward} \\ \hline
%\textbf{--}  &  \textbf{Na\"ive Baseline}	& \textbf{49.50} &	\textbf{-0.01956}  \\ \hline
1  &  Hitachi  & 0.6743 & 0.2988 \\ \hline
2  &  Amobee  & 0.6606 & 0.2766 \\ \hline
3  &  YNU-HPCC  & 0.6591 & 0.2783 \\ \hline
4  &  LMML  & 0.6469 & 0.2601 \\ \hline
5  &  XSYSIGMA  & 0.6446 & 0.2541 \\ \hline
6  &  ECNU  & 0.6438 & 0.2508 \\ \hline
7  &  Fermi  & 0.6393 & 0.2438 \\ \hline
8  &  zxchen  & 0.6347 & 0.2399 \\ \hline
9  &  Duluth  & 0.6320 & 0.2429 \\ \hline
10  &  WMD  & 0.6294 & 0.2291 \\ \hline
11  &  Buhscitu  & 0.6271 & 0.2190 \\ \hline
12  &  MLEngineer  & 0.6229 & 0.2046 \\ \hline
13  &  LRG  & 0.6218 & 0.2077 \\ \hline
14  &  UniTuebingenCL  & 0.6183 & 0.2110 \\ \hline
15  &  O698  & 0.6134 & 0.1954 \\ \hline
16  &  JUST\_Farah  & 0.6088 & 0.1841 \\ \hline
17  &  INGEOTEC  & 0.6050 & 0.1779 \\ \hline
18  &  Ferryman  & 0.6027 & 0.1771 \\ \hline
19  &  UPB  & 0.6001 & 0.1772 \\ \hline
20  &  Hasyarasa  & 0.5970 & 0.1673 \\ \hline
21  &  JokeMeter  & 0.5776 & 0.1487 \\ \hline
22  &  UTFPR  & 0.5696 & 0.1181 \\ \hline
23  &  Hahackathon  & 0.5426 & 0.0747 \\ \hline
24  &  SSN\_NLP  & 0.5377 & 0.0622 \\ \hline
25  &  WUY  & 0.5320 & 0.1113 \\ \hline
26  &  uir  & 0.5213 & 0.0567 \\ \hline
27  &  KdeHumor  & 0.5190 & 0.0272 \\ \hline
28  &  Titowak  & 0.5038 & -0.0021 \\ \hline
\textbf{--}  &  \textbf{Na\"ive Baseline}	& \textbf{0.4950} &	\textbf{-0.0196}  \\ \hline
29  &  heidy  & 0.4197 & -0.0995 \\ \hline
30  &  SO  & 0.3291 & -0.2064 \\ \hline
31  &  HumorAAC  & 0.3204 & -0.2177 \\ \hline

    \end{tabular}}
    %\end{adjustbox}}
    \caption{Official results for Subtask 2.}
    \label{tab:res-B}
\end{wraptable}

\nh{Why correlations for low-performing teams in Subtask 1 are unusually high?}

==> outline.tex <==
\begin{abstract}
    
\end{abstract}

\section{Introduction}
Give examples of how the data looks like. Table similar to funny headline example table in FunLines or NAACL, then quickly describe in text the dataset structure.

Goal of this task

Explain why humor is important and why we're doing this contest.

\nh{Can say results were promising..}

Talk about the large number of participants, especially compared to previous humor tasks.

\nh{Motivate: Detecting humor is a great AI test}


\section{Background}
This is best place to discuss our past papers and related work. We can make Background subsection in intro, or just put the related work in intro. 

Other humor detection papers, e.g. funny tweets. How this new contest is an evolution of previous work and how it advances the field in a smart way.

\section{Task Description}
Say, the objective is to build systems for understanding and recognizing humor. Dont justify why we are doing it, why 2 subtasks. Say, applications include humor generation.
\subsection{Task A: Funniness Regression}
Mention, motivate and justify evaluation/scoring criteria, i.e. why they are appropriate for these/humor tasks. Boldface or subsubsection for easy finding of evaluation metric.
\subsection{Task B: Funnier of the Two}
Mention evaluation criteria.

Discuss how Task B helps. Why add Task B in addition to Task A?

 

\section{Dataset}
Dataset~\cite{hossain-etal-2019-president}. Cite FunLines. Here are some quick insights into these datasets. Describe counts of train, dev, test examples. Mention that the datasets are different. 

Funniness frequency bins, mean, median. Discussion of length as function of funniness?

Talk about annotation differences between NAACL 2019 and FunLines.

For more details on these data, see NAACL 2019 and FunLines papers.
%\subsection{Data Analysis}

Data description: Annotation guidelines/procedure, summary statistics, refer to Figure 1 providing examples. Quality control. Summarize NAACL paper dataset section. Headline collection and sampling, source, time stamps.

\section{Participating Systems}
Nabil cluster the google docs into groups: pre-trained models, external data used?, ...

\subsection{Theories of Humor used by Systems}
Were they useful, or black box worked just as well or better?

\section{Evaluation}
Be aware of page limits, listing tables might take up lot of space.

\subsection{Baselines}
Task 1: mean training grade. LSTM using only edited headlines. BERT using only edited headlines. BERT using original and edited headlines. Report hyperparameter settings.

Task 2: majority training label.

\nh{Should there be a Data Analysis subsection here or under Analysis section?}
\subsection{Results}
Table of results. Then state which systems did well and how systems ranked.

\section{Analysis}
\nh{Analyze to show: where humor detection is difficult, which are the easy test cases, what the current models are struggling against and doing very good at}

Analyze all aggregate classification accuracy from all systems for each test set example.

Interesting aggregate visualizations of system performances. We can use many other evaluation metrics in addition to RMSE (e.g. correlation) and classification accuracy (Precision, Recall, F1). Also describe performance for top and bottom X\% of the data (X=10,20,30,40).

Error analysis.

\nh{Our goal is to do the kind of analysis so that we can provide as much insight as possible into humor generation in the dataset}

\nh{Here is our chance to impress readers with our data analysis and visualization skills.}

\subsection{Qualitative}
Top and bottom 5 headlines where all systems got correct. Where to focus more, Task A or B? Group analysis by model type (e.g. BERT vs LSTM)? How additional training data gives better classification.
\subsection{Quantitative}

\section{Discussion}
\subsection{Quirks on the Data}
\subsection{Benefits of using External Data}
\subsection{Lessons Learned}
(1) best way to detect humor
(2) best way to run a contest like ours - what would we do differently that is unique to humor detection.



%\section{Related Work}

\section{Conclusion}
Lessons learned, advice for future work on humor data collection and launching humor tasks. 

This is where we take a leadership position, influence and shape the future of humor research.

\section*{Acknowledgments}
Acknowledge participants and their hard work in advancing humor research?

==> tables.tex <==
\begin{wraptable}[50]{r}{0.36\textwidth} %[13] %[50]
    \centering
    \raisebox{0pt}[\dimexpr\height-0\baselineskip\relax]{
    \resizebox{0.355\textwidth}{!}{
    \begin{tabular}{|c|l|c|}
    \textbf{Rank}  & \textbf{Team}   & \textbf{RMSE} \\ \hline
    %\textbf{--} & \textbf{Na\"ive Baseline} & \textbf{0.57471} & \textbf{0.98616} & \textbf{0.83064} & \textbf{0.72266}	& \textbf{0.64004} & \textbf{0.00723} \\ \hline 

1  &  Hitachi  &  0.49725 \\ \hline
2  &  Amobee  &  0.50726 \\ \hline
3  &  YNU-HPCC  &  0.51737 \\ \hline
4  &  MLEngineer  &  0.51966 \\ \hline
5  &  LMML  &  0.52027 \\ \hline
6  &  ECNU  &  0.52187 \\ \hline
\textbf{--} & \textbf{RoBERTa} & \textbf{0.52207} \\ \hline 
7  &  LT3  &  0.52532 \\ \hline
8  &  WMD  &  0.52603 \\ \hline
9  &  Ferryman  &  0.52776 \\ \hline
10  &  zxchen  &  0.52886 \\ \hline
\textbf{--} & \textbf{BERT} & \textbf{0.53036} \\ \hline 
11  &  Duluth  &  0.53108 \\ \hline
12  &  will\_go  &  0.53228 \\ \hline
13  &  XSYSIGMA  &  0.53308 \\ \hline
14  &  LRG  &  0.53318 \\ \hline
15  &  MeisterMorxrc  &  0.53383 \\ \hline
16  &  JUST\_Farah  &  0.53396 \\ \hline
17  &  Lunex  &  0.53518 \\ \hline
18  &  unituebingenCL  &  0.53954 \\ \hline
\textbf{--} & \textbf{CBOW} & \textbf{0.54242} \\ \hline 
19  &  IRLab\_DAIICT  &  0.54670 \\ \hline
20  &  O698  &  0.54754 \\ \hline
21  &  UPB  &  0.54803 \\ \hline
22  &  Buhscitu  &  0.55115 \\ \hline
23  &  Fermi  &  0.55226 \\ \hline
24  &  INGEOTEC  &  0.55391 \\ \hline
25  &  JokeMeter  &  0.55791 \\ \hline
26  &  testing  &  0.55838 \\ \hline
27  &  HumorAAC  &  0.56454 \\ \hline
28  &  ELMo-NB  &  0.56829 \\ \hline
29  &  prateekgupta2533  &  0.56983 \\ \hline
30  &  funny3  &  0.57237 \\ \hline
31  &  WUY  &  0.57369 \\ \hline
32  &  XTHL  &  0.57470 \\ \hline
\textbf{--} & \textbf{BASELINE} & \textbf{0.57471} \\ \hline 
33  &  HWMT\_Squad  &  0.57471 \\ \hline
34  &  moonalasad  &  0.57479 \\ \hline
35  &  dianehu  &  0.57488 \\ \hline
36  &  Warren  &  0.57527 \\ \hline
37  &  tangmen  &  0.57768 \\ \hline
38  &  Lijunyi  &  0.57946 \\ \hline
39  &  Titowak  &  0.58157 \\ \hline
40  &  xenia  &  0.58286 \\ \hline
41  &  Hahackathon  &  0.59202 \\ \hline
42  &  KdeHumor  &  0.61643 \\ \hline
43  &  uir  &  0.62401 \\ \hline
44  &  SO  &  0.65099 \\ \hline
45  &  heidy  &  0.68338 \\ \hline
46  &  Hasyarasa  &  0.70333 \\ \hline
47  &  frietz58  &  0.72252 \\ \hline
48  &  SSN\_NLP  &  0.84476 \\ \hline
    \end{tabular}}}
    \caption{Official results for Subtask 1.}
    \label{tab:res-A}
\end{wraptable}


==> unused.tex <==
%\jk{It's a nice figure, but I don't think it really gives much insight.} \nh{To John: then lets make this point while explaining Fig 4(b)}
%Figure~\ref{fig:task1-aggregate-error} shows the histogram of errors of the aggregate top 20 systems. This is similar to a skewed normal distribution. \nh{Useless figure?}
\begin{wrapfigure}{r}{8.2cm}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c}
        \includegraphics{figures/aggregate-error-task1.png}
    \end{tabular}}
    \caption{Normalized frequency histogram of top 20 systems' aggregate error values, shaped like a skewed normal distribution. \nh{should we remove it?} \jk{I vote to remove.}}
    \label{fig:task1-aggregate-error}
\end{wrapfigure}


